INACIA: Integrating Large Language Models in Brazilian Audit Courts: Opportunities and Challenges

This paper introduces INACIA (Instru\c{c}\~ao Assistida com Intelig\^encia Artificial), a groundbreaking system designed to integrate Large Language Models (LLMs) into the operational framework of Brazilian Federal Court of Accounts (TCU). The system automates various stages of case analysis, including basic information extraction, admissibility examination, Periculum in mora and Fumus boni iuris analyses, and recommendations generation. Through a series of experiments, we demonstrate INACIA's potential in extracting relevant information from case documents, evaluating its legal plausibility, and formulating propositions for judicial decision-making. Utilizing a validation dataset alongside LLMs, our evaluation methodology presents a novel approach to assessing system performance, correlating highly with human judgment. These results underscore INACIA's potential in complex legal task handling while also acknowledging the current limitations. This study discusses possible improvements and the broader implications of applying AI in legal contexts, suggesting that INACIA represents a significant step towards integrating AI in legal systems globally, albeit with cautious optimism grounded in the empirical findings.

==> tables/check_list_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\caption{Results of the allegations and requests extraction using the checklist approach.} 
\label{tab:check_eval_results}
\begin{tabular}{@{}lccc@{}}
\toprule
     & Precision & Recall & F1    \\ \midrule
Mean & 0.693     & 0.500  & 0.532 \\
Std  & 0.263     & 0.224  & 0.187 \\
Min  & 0.100     & 0.000  & 0.000 \\
Max  & 1.000     & 1.000  & 1.000 \\ \bottomrule
\end{tabular}
\end{table}
